Unleashing the Power of T1-cells in SFQ Arithmetic Circuits

Rapid single-flux quantum (RSFQ), a leading cryogenic superconductive electronics (SCE) technology, offers extremely low power dissipation and high speed. However, implementing RSFQ systems at VLSI complexity faces challenges, such as substantial area overhead from gate-level pipelining and path balancing, exacerbated by RSFQ's limited layout density. T1 flip-flop (T1-FF) is an RSFQ logic cell operating as a pulse counter. Using T1-FF the full adder function can be realized with only 40% of the area required by the conventional realization. This cell however imposes complex constraints on input signal timing, complicating its use. Multiphase clocking has been recently proposed to alleviate gate-level pipelining overhead. The fanin signals can be efficiently controlled using multiphase clocking. We present the novel two-stage SFQ technology mapping methodology supporting the T1-FF. Compatible parts of the SFQ network are first replaced by the efficient T1-FFs. Multiphase retiming is next applied to assign clock phases to each logic gate and insert DFFs to satisfy the input timing. Using our flow, the area of the SFQ networks is reduced, on average, by 6% with up to 25% reduction in optimizing the 128-bit adder.

==> table_dcm.tex <==
\begin{table}[h]
\setlength\tabcolsep{2pt}
\centering
\caption{Comparison of multiphase clocking with dual clocking method \cite{dual_clock} with 20\% throughput}
\begin{tabular}{r|rrr|rrr|r}
\toprule 
          & \multicolumn{3}{c|}{Multiphase (our work)}                                      & \multicolumn{3}{c|}{Dual clocking method \cite{dual_clock}}  &              \\
\cmidrule(rl){1-1} \cmidrule(rl){2-4} \cmidrule(rl){5-7} \cmidrule(rl){8-8}
          & \multicolumn{1}{r|}{DFF}   & \multicolumn{1}{r|}{JJ}     & \hsc{Latency} & \multicolumn{1}{r|}{DFF}   & \multicolumn{1}{r|}{NDRO} & \hsc{Latency} & Impr. \% \\
\cmidrule(rl){1-1} \cmidrule(rl){2-4} \cmidrule(rl){5-7} \cmidrule(rl){8-8}
\cf{sin}       & \multicolumn{1}{r|}{11,170} & \multicolumn{1}{r|}{121,350} & 17      & \multicolumn{1}{r|}{13,581} & \multicolumn{1}{r|}{24}   & 186   & 17.8      \\
\rowcolor{gray!15}
\cf{int2float} & \multicolumn{1}{r|}{258}   & \multicolumn{1}{r|}{4,239}   & 2       & \multicolumn{1}{r|}{139}   & \multicolumn{1}{r|}{11}   & 16    & -85.6     \\
\cf{priority}  & \multicolumn{1}{r|}{7,567}  & \multicolumn{1}{r|}{62,490}  & 17      & \multicolumn{1}{r|}{21,115} & \multicolumn{1}{r|}{128}  & 249   & 64.2      \\
\rowcolor{gray!15}
\cf{i2c}       & \multicolumn{1}{r|}{1,208}  & \multicolumn{1}{r|}{21,663}  & 3       & \multicolumn{1}{r|}{1,544}  & \multicolumn{1}{r|}{147}  & 17    & 21.8      \\
\cf{voter}     & \multicolumn{1}{r|}{4,353}  & \multicolumn{1}{r|}{147,638} & 8       & \multicolumn{1}{r|}{6,716}  & \multicolumn{1}{r|}{1,001} & 71    & 35.2      \\
\rowcolor{gray!15}
\cf{c432}      & \multicolumn{1}{r|}{443}   & \multicolumn{1}{r|}{4,555}   & 4       & \multicolumn{1}{r|}{447}   & \multicolumn{1}{r|}{36}   & 24    & 0.9       \\
\cf{c499}      & \multicolumn{1}{r|}{242}   & \multicolumn{1}{r|}{4,691}   & 2       & \multicolumn{1}{r|}{218}   & \multicolumn{1}{r|}{41}   & 13    & -11.0     \\
\rowcolor{gray!15}
\cf{c1908}     & \multicolumn{1}{r|}{212}   & \multicolumn{1}{r|}{3,593}   & 3       & \multicolumn{1}{r|}{473}   & \multicolumn{1}{r|}{33}   & 20    & 55.2      \\
\cf{c3540}     & \multicolumn{1}{r|}{812}   & \multicolumn{1}{r|}{14,456}  & 4       & \multicolumn{1}{r|}{795}   & \multicolumn{1}{r|}{50}   & 32    & -2.1      \\
\rowcolor{gray!15}
\cf{c5315}     & \multicolumn{1}{r|}{1,050}  & \multicolumn{1}{r|}{22,735}  & 3       & \multicolumn{1}{r|}{2,554}  & \multicolumn{1}{r|}{178}  & 27    & 58.9      \\
\cf{c7552}     & \multicolumn{1}{r|}{847}   & \multicolumn{1}{r|}{17,722}  & 4       & \multicolumn{1}{r|}{1,912}  & \multicolumn{1}{r|}{207}  & 21    & 55.7      \\
\rowcolor{gray!15}
\multicolumn{1}{r}{Average}   & \multicolumn{1}{r}{}      & \multicolumn{1}{r}{}       &    \multicolumn{1}{r}{}     & \multicolumn{1}{r}{}      & \multicolumn{1}{r}{}     &      & 19.2      \\
\bottomrule
\end{tabular}\label{tab:with_dcm}
\end{table}

% \hsc{benchmark} & \hsc{\#DFF} & \hsc{\#JJ}    & \hsc{Depth} & \hsc{\#DFF} & \hsc{Impr.} & \hsc{\#JJ} & \hsc{Impr.} & \hsc{Depth} & \hsc{Impr.} & \hsc{Runtime, s} \\

==> table_dcm_2.tex <==
\begin{table*}[h]
\setlength\tabcolsep{4pt}
\centering
\caption{Comparison of multiphase clocking with dual clocking method \cite{dual_clock} for different throughputs}
\vspace{-1em}
\begin{tabular}{l|rrrrrr|rrrrrr}
               & \mcl{6}{c|}{1/7 throughput}                                                              & \mcl{6}{c}{1/12 throughput}                                                                 \\
\cmidrule(rl){2-7} \cmidrule(rl){8-13}
               & \mcl{2}{c}{DCM}                 & \mcl{2}{c}{Multiphase}           & \mcl{2}{c|}{Change}  & \mcl{2}{c}{DCM}                    & \mcl{2}{c}{Multiphase}          & \mcl{2}{c}{Change}    \\
               & \#DFF  & \#JJ                   & \#DFF   & \#JJ                   & \#DFF    & \#JJ     & \#DFF     & \#JJ                   & \#DFF  & \#JJ                   & \#DFF     & \#JJ     \\
\cmidrule(rl){2-3} \cmidrule(rl){4-5} \cmidrule(rl){6-7} \cmidrule(rl){8-9} \cmidrule(rl){10-11} \cmidrule(rl){12-13}
\cf{int2float} & 117    & \mcl{1}{r|}{7'770}     & 217     & \mcl{1}{r|}{5'136}     & +85.47\% &--33.90\% & 39        & \mcl{1}{r|}{5'140}     & 46     & \mcl{1}{r|}{3'939}     & +17.95\%  &--23.37\% \\
\rowcolor{gray!15}
\cf{priority}  & 8'562  & \mcl{1}{r|}{257'252}   & 3'285   & \mcl{1}{r|}{45'094}    &--61.63\% &--82.47\% & 4'225     & \mcl{1}{r|}{158'568}   & 1'775  & \mcl{1}{r|}{34'524}    &--57.99\%  &--78.23\% \\
\cf{voter}     & 7'204  & \mcl{1}{r|}{447'044}   & 2'180   & \mcl{1}{r|}{162'804}   &--69.74\% &--63.58\% & 3'732     & \mcl{1}{r|}{355'144}   & 1'568  & \mcl{1}{r|}{158'520}   &--57.98\%  &--55.36\% \\
\rowcolor{gray!15}
\cf{c432}      & 224    & \mcl{1}{r|}{10'734}    & 342     & \mcl{1}{r|}{5'116}     & +52.68\% &--52.34\% & 118       & \mcl{1}{r|}{7'124}     & 240    & \mcl{1}{r|}{4'402}     & +103.39\% &--38.21\% \\
\cf{c880}      & 362    & \mcl{1}{r|}{14'658}    & 254     & \mcl{1}{r|}{6'190}     &--29.83\% &--57.77\% & 187       & \mcl{1}{r|}{9'483}     & 119    & \mcl{1}{r|}{5'245}     &--36.36\%  &--44.69\% \\
\rowcolor{gray!15}
\cf{c1908}     & 282    & \mcl{1}{r|}{13'169}    & 125     & \mcl{1}{r|}{3'529}     &--55.67\% &--73.20\% & 144       & \mcl{1}{r|}{8'739}     & 69     & \mcl{1}{r|}{3'137}     &--52.08\%  &--64.10\% \\
\cf{c3540}     & 776    & \mcl{1}{r|}{43'437}    & 589     & \mcl{1}{r|}{17'016}    &--24.10\% &--60.83\% & 282       & \mcl{1}{r|}{26'897}    & 440    & \mcl{1}{r|}{15'973}    & +56.03\%  &--40.61\% \\
\rowcolor{gray!15}
\cf{c1355}     & 193    & \mcl{1}{r|}{8'739}     & 46      & \mcl{1}{r|}{4'515}     &--76.17\% &--48.34\% & 119       & \mcl{1}{r|}{6'149}     & 44     & \mcl{1}{r|}{4'501}     &--63.03\%  &--26.80\% \\
\cf{s13207}    & 1'795  & \mcl{1}{r|}{106'346}   & 1'837   & \mcl{1}{r|}{42'382}    & +2.34\%  &--60.15\% & 571       & \mcl{1}{r|}{60'766}    & 1'082  & \mcl{1}{r|}{37'097}    & +89.49\%  &--38.95\% \\
\rowcolor{gray!15}
\cf{s5378}     & 645    & \mcl{1}{r|}{50'766}    & 808     & \mcl{1}{r|}{21'761}    & +25.27\% &--57.13\% & 255       & \mcl{1}{r|}{34'053}    & 368    & \mcl{1}{r|}{18'681}    & +44.31\%  &--45.14\% \\
\cf{s382}      & 56     & \mcl{1}{r|}{4'448}     & 89      & \mcl{1}{r|}{2'411}     & +58.93\% &--45.80\% & 9         & \mcl{1}{r|}{2'750}     & 48     & \mcl{1}{r|}{2'124}     & +433.33\% &--22.76\% \\
\cmidrule(rl){1-1} \cmidrule(rl){2-7} \cmidrule(rl){8-13}
Geomean        & 557.04 & \mcl{1}{r|}{29'868.20} & 413.48  & \mcl{1}{r|}{11'965.54} &--25.77\% &--59.94\% & 227.85    & \mcl{1}{r|}{19'565.38} & 229.57 & \mcl{1}{r|}{10'467.10} & +0.76\%   &--46.50\% 
\end{tabular}\label{tab:with_dcm}
\end{table*}

==> table_ext_abstract.tex <==
\begin{table*}
\centering
% \textwidth
% \adjustbox{\textwidth}{
% \begin{adjustbox}{width=\textwidth}{
\caption{Multiphase clocking with T1 cells applied to a subset of EPFL and ISCAS benchmark circuits }
\label{tab:results}
% \resizebox{\textwidth}{!}{
\begin{tabular}{l||rr||rrr|rr||rrr|rr}
\toprule
 & \multicolumn{2}{c||}{T1 cells} & \multicolumn{3}{c|}{Area} & \multicolumn{2}{c||}{Ratio vs.} & \multicolumn{3}{c|}{Depth} & \multicolumn{2}{c}{Ratio vs.}\\
% \cmidrule(rl){1-1} \cmidrule(rl){2-2}  \cmidrule(rl){3-5}  \cmidrule(rl){6-7} \cmidrule(rl){8-10}  \cmidrule(rl){11-12} \cmidrule(rl){13-15}  \cmidrule(rl){16-17} 
benchmark & found & used & 1$\mathgtt{f}$ & 4$\mathgtt{f}$ & T1 & 1$\mathgtt{f}$ & 4$\mathgtt{f}$ & 1$\mathgtt{f}$ & 4$\mathgtt{f}$ & T1 & 1$\mathgtt{f}$ & 4$\mathgtt{f}$\\
\cmidrule(rl){1-1} \cmidrule(rl){2-3}  \cmidrule(rl){4-6}  \cmidrule(rl){7-8} \cmidrule(rl){9-11}  \cmidrule(rl){12-13} 
\mtt{adder} & 127	&	127     & 238'419 & 64'784 & 48'844 & 0.20 & 0.75 & 128 & 32 & 33 & 0.26 & 1.03 \\
\rowcolor{gray!15}
\mtt{sin}   & 81	&	77      & 164'938 & 103'443 & 102'806 & 0.62 & 0.99 & 88 & 22 & 25 & 0.28 & 1.14 \\
\mtt{voter} & 252	&	252     & 222'101 & 187'997 & 182'972 & 0.82 & 0.97 & 38 & 10 & 11 & 0.29 & 1.10 \\
\rowcolor{gray!15}
\mtt{square} & 861	&	806     & 525'311 & 329'101 & 301'287 & 0.57 & 0.92 & 126 & 32 & 32 & 0.25 & 1.00 \\
\mtt{multiplier} & 824	&	769 & 682'792 & 374'260 & 356'984 & 0.52 & 0.95 & 136 & 33 & 36 & 0.26 & 1.09 \\
\rowcolor{gray!15}
\mtt{log2} & 644	&	593     & 978'178 & 605'813 & 598'292 & 0.61 & 0.99 & 160 & 40 & 47 & 0.29 & 1.18 \\
\cmidrule(rl){1-1} \cmidrule(rl){2-3}  \cmidrule(rl){4-6}  \cmidrule(rl){7-8} \cmidrule(rl){9-11}  \cmidrule(rl){12-13} 
\rowcolor{gray!30}
% \multicolumn{6}{l}{Average}& 0.35 & \multicolumn{1}{l}{0.94} & \multicolumn{3}{l}{} & 0.59 & \multicolumn{1}{l}{0.94} & \multicolumn{3}{l}{} & 0.29 & 1.13\\
\bottomrule
\end{tabular}
% }
\end{table*}

